Detection of periodic radio signal from the blazar J1043+2408

Search for periodic signals from blazars has become widely discussed topic in recent years. In the scenario that such periodic changes originate from the innermost regions of blazars, the signals bear imprints of the processes occurring near the central engine, which is mostly inaccessible to our direct view. Such signals provide insights into various aspect of blazar studies including disk-jet connection, magnetic field configuration and, more importantly, strong gravity near the supermassive black holes and release of gravitational waves from the binary supermassive black hole systems. In this work, we report detection of a periodic signal in the radio light curve of the blazar J1043+2408 spanning $\sim$10.5 years. We performed multiple methods of time series analysis, namely, epoch folding, Lomb-Scargle periodogram, and discrete auto-correlation function. All three methods consistently reveal a repeating signal with a periodicity of $\sim560$ days. To robustly account for the red-noise processes usually dominant in the blazar variability and other possible artifacts, a large number of Monte Carlo simulations were performed. This allowed us to estimate a high significance (99.9\% local and 99.4\% global) against possible spurious detection. As possible explanations, we discuss a number of scenarios including binary supermassive black hole system, Lense-Thirring precession and jet precession.

==> citations.tex <==
 \bibitem{Meier12} Meier, D.~L.\ ,
 Black Hole Astrophysics: The Engine Paradigm, Springer, Verlag Berlin Heidelberg, 
{\bf 2012}

\bibitem{Bhatta2017} 
 Bhatta, G.,\
 Radio and $\gamma$-Ray Variability in the BL Lac PKS  $0219-164$: Detection of Quasi-periodic Oscillations in the Radio Light Curve,  {\em ApJ}, {\bf 2017}, 487, 7B

 \bibitem{Bhatta2016b}  
 Bhatta, G., Zola S., Stawarz, L., et al.\ 
Detection of Possible Quasi-periodic Oscillations in the Long-term Optical Light Curve of the BL Lac Object OJ 287, 
{\em ApJ}, {\bf 2016}, 832, 47


\bibitem{Zola2016} Zola, S., Valtonen, M., Bhatta, G., et al.\
A Search for QPOs in the Blazar OJ287: Preliminary Results from the 2015/2016 Observing Campaign
{\em Galaxies}, {\bf 2016}, 4, 41

\bibitem{MG85}
Marscher, A.~P., \& Gear, W.~K.\
{Models for high-frequency radio outbursts in extragalactic sources, with application to the early 1983 millimeter-to-infrared flare of 3C 273}.  {\em ApJ} {\bf 1985}, 298, 114 

\bibitem{Camenzind92} 
{The lighthouse effect of relativistic jets in blazars - A geometric origin of intraday variability}
Camenzind, M., \& Krockenberger, M.\ {\em A\&A} {\bf 1992}, 255, 59 

\bibitem{Wagner95}
Wagner, S.~J., \& Witzel, A.
{Intraday Variability In Quasars and BL Lac Objects}, {\em ARAA} {\bf 1995},  33, 163

\bibitem{bhatta013}
{Bhatta G., Webb J. R, and Hollingsworth H. et al.} The 72-h WEBT microvariability observation of blazar S5 0716 + 714 in 2009. {\em A\&A} {\bf 2008}, 558, A92.

\bibitem{Quirrenbach1992} Quirrenbach, A., Witzel, A., Kirchbaum, T.~P., et al.\ 
Statistics of intraday variability in extragalactic radio sources
{\bf 1992}, {\em A\&A},  258, 279

\bibitem{Heidt1996} Heidt, J., \& Wagner, S.~J.\ 
Statistics of optical intraday variability in a complete sample of radio-selected BL Lacertae objects,
{\bf 1996}, {\em A\&A},  305, 42

\bibitem{Bai1998} Bai, J.~M., Xie, G.~Z., Li, K.~H., Zhang, X., \& Liu, W.~W.\ 
The intraday variability in the radio-selected and X-ray-selected BL Lacertae objects
{\bf 1998}, {\em A\&AS},  132, 83

\bibitem{Kraus2003} Kraus, A., Krichbaum, T.~P., Wegner, R., et al.\  
Intraday variability in compact extragalactic radio sources. II. Observations with the Effelsberg 100 m radio telescope
{\bf 2003}, {\em A\&A}, 401, 161

\bibitem{Howard2004} Howard, E.~S., Webb, J.~R., Pollock, J.~T., \& Stencel, R.~E.\ 
Microvariability and Long-Term Variability of Four Blazars
{\bf 2004}, {\em AJ}, 127, 17

\bibitem{Rani2011} Rani, B., Gupta, A.~C., Joshi, U.~C., Ganesh, S., \& Wiita, P.~J.\ 
Optical intraday variability studies of 10 low energy peaked blazars
{\bf 2011}, {\em MNRAS}, 413, 2157

\bibitem{Gaur2012} Gaur, H., Gupta, A.~C., Strigachev, A., et al.\  
Optical flux and spectral variability of blazars
{\em MNRAS}, {\bf 2012}, 425, 3002

\bibitem{Bachev2012} Bachev, R., Semkov, E., Strigachev, A., et al.\ 
The nature of the intra-night optical variability in blazars
{\em MNRAS}, {\bf 2012}, 424, 2625

\bibitem{Guo2016} {{Guo}, Y.~C. and {Hu}, S.~M. and {Li}, Y.~T. and {Chen}, X.}
Statistical analysis of the temporal properties of BL Lacertae,
{\em MNRAS}, {\bf 2016}, 460, 1790


 %Reference 1

\bibitem{bhatta015}
Bhatta, G., et al.\
Discovery of a Highly Polarized Optical Microflare in Blazar S5 0716+714 during the 2014 WEBT Campaign. {\em ApJ} {\bf 2015} 809L, 27B

\bibitem{bhatta016}
Bhatta, G., Stawarz, L., Ostrowski, M., et al. 
Multifrequency Photo-polarimetric WEBT Observation Campaign on the Blazar S5 0716+714: Source Microvariability and Search for Characteristic Timescales 
{\em ApJ} {\bf 2016}, 831, 92B

 \bibitem{Bhatta2016a} 
 Bhatta, G.,\
Investigating the Innermost Jet Structures of Blazar S5 0716+714 Using Uniquely Dense Intra-day Photo-polarimetric Observations, 
{\em Galaxies}, {\bf 2016} 4, 56 




\bibitem{Bhatta2017b}Bhatta G., Mohorian, M., and Bilinsky, I.
Hard X-ray Properties of NuSTAR Blazars
ApJ submitted; http://arxiv.org/abs/1710.09910


\bibitem{Wehrle2016} Wehrle, A.~E., Grupe, D., Jorstad, S.~G., et al.\ 
Erratic Flaring of BL Lac in 2012-2013: Multiwavelength Observations
{\bf 2016}, {\em ApJ}, 816, 53

\bibitem{Raiteri2013} Raiteri, C.~M., Villata, M., D'Ammando, F., et al.\ 
The awakening of BL Lacertae: observations by Fermi, Swift and the GASP-WEBT
{\bf 2013}, {\em MNRAS}, 436, 1530

\bibitem{Raiteri2010} Raiteri, C.~M., Villata, M., Bruschini, L., et al.\ 
Another look at the BL Lacertae flux and spectral variability. Observations by GASP-WEBT, XMM-Newton, and Swift in 2008-2009
 {\bf 2010}, {\em A\&A}, 524, A43

\bibitem{Villata2009} Villata, M., Raiteri, C.~M., Larionov, V.~M., et al.\	
The correlated optical and radio variability of BL Lacertae. WEBT data analysis 1994-2005,
{\bf 2009}, {\em A\&A},  501, 455

\bibitem{Bottcher2003} B{\"o}ttcher, M., Marscher, A.~P., Ravasio, M., et al.\ 
Coordinated Multiwavelength Observations of BL Lacertae in 2000,
{\bf 2003}, {\em ApJ}, 596, 847


\bibitem{Speziali1998} Speziali, R., \& Natali, G.\ 
BVI microvariability in BL Lacertae during the summer 1997 outburst
{\bf 1998}, {\em A\&A},  339, 382

\bibitem{Massaro1998} Massaro, E., Nesci, R., Maesano, M., Montagni, F., \& D'Alessio, F.\ 
Fast variability of BL Lacertae at 1mum
{\bf 1998}, {\em MNRAS}, 299, 47

\bibitem{Nesci1998} Nesci, R., Maesano, M., Massaro, E., et al.\ 
Intraday variability of BL Lacertae in the great 1997 outburst
{\bf 1998}, {\em A\&A},  332, L1

\bibitem{Clements2001} Clements, S.~D., \& Carini, M.~T.\ 
Multiband Microvariability Observations of BL Lacertae during the Outburst of 1997
{\bf 2001}, {\em AJ},  121, 90

\bibitem{Zhai2012} Zhai, M., \& Wei, J.~Y.\
Intra-night optical multiband variability of BL Lacertae during the 2011 outburst
{\bf 2012}, {\em A\&A}, 538, A125

\bibitem{Agarwal2015} Agarwal, A., \& Gupta, A.~C. 
Multiband optical variability studies of BL Lacertae
{\bf 2015}, {\em MNRAS}, 450, 541

\bibitem{Gaur2015} Gaur, H., Gupta, A.~C., Bachev, R., et al.\ 
Nature of intranight optical variability of BL Lacertae
{\bf 2015}, {\em MNRAS}, 452, 4263




\bibitem{Papadakis2003} Papadakis, I.~E., Boumis, P., Samaritakis, V., \& Papamastorakis, J.\ 
Multi-band optical micro-variability observations of BL Lacertae
{\bf 2003}, {\em A\&A},  397, 565

\bibitem{Villata2004} Villata, M., Raiteri, C.~M., Aller, H.~D., et al.\ 
The WEBT campaigns on BL Lacertae. Time and cross-correlation analysis of optical and radio light curves 1968-2003
{\bf 2004}, {\em A\&A},  424, 497

\bibitem{Abdo2011} Abdo, A.~A., Ackermann, M., Ajello, M., et al.\ 
The First Fermi Multifrequency Campaign on BL Lacertae: Characterizing the Low-activity State of the Eponymous Blazar
{\bf 2011}, {\em ApJ}, 730, 101

\bibitem{Cohen2015} Cohen, M.~H., Meier, D.~L., Arshakian, T.~G., et al.
Studies of the Jet in Bl Lacertae. II. Superluminal Alfvén Waves
{\bf 2015}, {\em ApJ}, 803, 3


\bibitem{Marscher2008} Marscher, A.~P., Jorstad, S.~G., D'Arcangelo, F.~D., et al.\ 
The inner jet of an active galactic nucleus as revealed by a radio-to-$\gamma$-ray outburst
{\bf 2008}, {\em Nature}, 452, 966

\bibitem{Arlen2013} Arlen, T., Aune, T., Beilicke, M., et al.
Rapid TeV Gamma-Ray Flaring of BL Lacertae
{\em ApJ}, {\bf 2013} 762, 92

\bibitem{Gaur2014} Gaur, H., Gupta, A.~C., Wiita, P.~J., et al. 
Anti-correlated Optical Flux and Polarization Variability in BL Lac
 {\bf 2014}, {\em ApJL}, 781, L4

\bibitem{Webb2016} Webb, J.\ 
Multi-Frequency Blazar Micro-Variability as a Tool to Investigate Relativistic Jets
{\em Galaxies}, {\bf 2016}, 4, 15

\bibitem{Howell1988} Howell, S.~B., Warnock, A., III, \& Mitchell, K.~J.\ 
Statistical error analysis in CCD time-resolved photometry with applications to variable stars and quasars
{\bf 1988}, {\em AJ}, 95, 247

\bibitem{bessel98} Bessell, M. S., Castelli, F., \& Plez, B.\
Model atmospheres broad-band colors, bolometric corrections and temperature calibrations for O - M stars
{\em A\&A}, {\bf 1998} 333, 231

\bibitem{vau03}Vaughan, S., Edelson, R., Warwick, R. S., \& Uttley, P.
On characterizing the variability properties of X-ray light curves from active galaxies
 {\bf 2003}, {\em MNRAS}, 345, 1271

\bibitem{Aleksic2015} Aleksi{\'c}, J., Ansoldi, S., Antonelli, L.~A., et al.\ 
The 2009 multiwavelength campaign on Mrk 421: Variability and correlation studies
{\em A\&A}, {\bf 2015}, 576, A126

\bibitem{Zhang2013} Zhang, Y.-H., Bian, F.-Y., Li, J.-Z., \& Shang, R.-C.\ 
Optical observations of BL Lacertae in 2004-2005
 {\bf 2013}, {\em MNRAS}, 432, 1189

\bibitem{EK88}
 Edelson, R. A., \& Krolik, J. H.\ 
 The discrete correlation function - A new method for analyzing unevenly sampled variability data, 
{\em ApJ}, {\bf 1988} 333, 646

\bibitem{Abdo2010} Abdo, A.~A., Ackermann, M., Ajello, M., et al.\ 
Gamma-ray Light Curves and Variability of Bright Fermi-detected Blazars
 {\em ApJ}, {\bf 2010}, 722, 520 

\bibitem{Simonetti85}Simonetti J. H., Cordes J. M., Heeschen D. S.\ 
Flicker of extragalactic radio sources at two frequencies,
{\em ApJ}, {\bf 1985}, 704, L129

\bibitem{Hughes1992} Hughes, P.~A., Aller, H.~D., \& Aller, M.~F.\ 
The University of Michigan radio astronomy data base. I - Structure function analysis and the relation between BL Lacertae objects and quasi-stellar objects
{\em ApJ}, {\bf 1992}, 396, 469

%***************************************************************


\bibitem{Lainela1993} Lainela, M., \& Valtaoja, E.\ 1993,	
Structure Function Analysis of High Radio Frequency Variability in the Metsaehovi Monitoring Sample of Active Galactic Nuclei,
{\em ApJ}, {\bf 1993}, 416, 485

\bibitem{Paltani1997} Paltani, S., Courvoisier, T.~J.-L., Blecha, A., \& Bratschi, P.\ 
Very rapid optical variability of PKS 2155-304
{\em A\&A}, {\bf  1997}, 327, 539

\bibitem{Zhang02}Zhang, Y. H.
Four Years of Monitoring Blazar PKS 2155-304 with BeppoSAX: Probing the Dynamics of the Jet,
{\em ApJ}, {\bf 2002}, 572, 762

\bibitem{Emmanoulopoulos10}Emmanoulopoulos, D.; McHardy, I. M.; Uttley, P.
On the use of structure functions to study blazar variability: caveats and problems,
{\em MNRAS}, {\bf 2010}, 404, 931E

\bibitem{Narayan2012} Narayan, R., \& Piran, T.\ 
Variability in blazars: clues from PKS 2155-304
 {\bf 2012}, {\em MNRAS}, 420, 604

\bibitem{Marscher2014} Marscher, A.~P.\ 
Turbulent, Extreme Multi-zone Model for Simulating Flux and Polarization Variability in Blazars
{\em ApJ}, {\bf 2014}, 780, 87 

\bibitem{Fuhrmann2014} Fuhrmann, L., Larsson, S., Chiang, J., et al.\ 
Detection of significant cm to sub-mm band radio and $\gamma$-ray correlated variability in Fermi bright blazars
{\em MNRAS}, {\bf 2014}, 441, 1899


\bibitem{Mangalam1993} Mangalam, A.~V., \& Wiita, P.~J.\ 
Accretion disk models for optical and ultraviolet microvariability in active galactic nuclei
{\em ApJ}, {\bf 1993}, 406, 420

\bibitem{Hardee1999} Hardee, P.~E., \& Rosen, A.\ 
On the Dynamics and Structure of Three-dimensional Trans-Alfvénic Jets
{\em ApJ}, {\bf 1999}, 524, 650 

%Reference 2
\bibitem{Kirk098}
{{Kirk}, J.~G. and {Rieger}, F.~M. and {Mastichiadis}, A.} Particle acceleration and synchrotron emission in blazar jets.
{\em A\&A} {\bf 1998}, 333, 452K.
















